Generalization, Mayhems and Limits in Recurrent Proximal Policy Optimization

At first sight it may seem straightforward to use recurrent layers in Deep Reinforcement Learning algorithms to enable agents to make use of memory in the setting of partially observable environments. Starting from widely used Proximal Policy Optimization (PPO), we highlight vital details that one must get right when adding recurrence to achieve a correct and efficient implementation, namely: properly shaping the neural net's forward pass, arranging the training data, correspondingly selecting hidden states for sequence beginnings and masking paddings for loss computation. We further explore the limitations of recurrent PPO by benchmarking the contributed novel environments Mortar Mayhem and Searing Spotlights that challenge the agent's memory beyond solely capacity and distraction tasks. Remarkably, we can demonstrate a transition to strong generalization in Mortar Mayhem when scaling the number of training seeds, while the agent does not succeed on Searing Spotlights, which seems to be a tough challenge for memory-based agents.

==> content/bugs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Inhibiting Factors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Deep Reinforcement Learning algorithms in general are prone to bugs, that are difficult to trace.
Adding recurrent layers to the PPO model notably increases the complexity of the entire implementation.
While working on the baseline implementation, several bugs severely hindered progress.
Two of those are related to the utilized machine learning framework PyTorch.
Unintentionally feeding $None$ as hidden state to the recurrent layer causes the network to initialize hidden states as zero.
This bug causes gradients to explode.
Further, when feeding a recurrent layer, PyTorch expects the sequence length to be the first dimension of the fed data.
Naively reshaping the data causes a catastrophic shift.
This bug may be circumvented by setting the batch first argument of the recurrent layer's forward function to true.
Also, one has to note that the output of an LSTM or GRU cell is already activated.
Adding another activation, like ReLU, on top might hurt performance.
%At last, hidden states were unintentionally not re-initialized to zero.
%Hence, each new episode used the hidden state from the previous one.

==> content/discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussing Challenges in Searing Spotlights}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Searing Spotlights, the agent is asked to collect all coins, while not being unveiled by any of the moving spotlights.
The agent's observation seldomly encompasses information on the whereabouts of the coins and itself, because these are only visible during the beginning of the episode and while being spotted by a light.
Therefore, this important information has to be inferred from past observations, which should be taken care of by the agent's memory.
One strategy could be to ease memorizing the agent's position by moving continuously towards environment boundaries, because moving for long enough in one direction raises the confidence of being at the min or max position on one or both axes.
Another valid approach could be to trade-off between the spotlight's penalty and directly observing the agent's position.
The agent might intentionally risk being visible to reveal its position.

Recurrent PPO does not seem to find any policy to solve Searing Spotlights.
This can be due to the agent not being able to directly impact its observations for the most part of the episode, even though it perceives its last action.
So how should the agent be able to assign credit to its performed decisions?
The spotlights may worsen this dilemma by causing noise and distractions due to their stochastic behavior (random spawn positions and stochastic movement).
To gain more insights, the environment can be ablated using these simplifications:
\begin{compactitem}
    \item removing spotlight penalties (i.e. damage and reward)
    \item limiting the number of coins to one
    \item increasing the scale of the agent and the coin
    \item making the spotlights stationary
    \item making the agent or the coin permanently visible
\end{compactitem}
Applying the first two measures did not lead to successful training.
Scaling up the size of the agent and the coin by an order of two or three failed as well.
Once spotlights are stationary, the agent easily learns to collect the coin, but only when its scale is set to three\footnote{More figures, showing the scale of the agent and stationary spotlights, can be found in Appendix \ref{sec:simplifications}.}.
Lowering the scale to two does not always work out like before.
The original scale did not solve the task under stationary spotlights.
If the agent is scaled up and always visible, but the spotlights move, the task remains unsolved.
We did not explore all permutations of available simplifications yet, but it seems that moving spotlights are the toughest challenge in Searing Spotlights.
To overcome their threat of distraction, a completely different approach to recurrent PPO shall be considered.
We believe that a transformer architecture as episodic memory, like the Hierarchical Chunk Attention Memory \cite{Lampinen2021htm}, is more capable and robust to distractions.
Doing so, the agent could recall every single extracted feature from past observations to filter out spotlights and to better trace itself.
This, however, is left to future work.




==> tables/config_common.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{small}
\centering
\begin{tabular}{l|l}
\rowcolor[HTML]{D1D1D1} 
\textbf{Parameter} & \textbf{Value} \\ \hline
\rowcolor[HTML]{EFEFEF} 
Discount Factor             & 0.99           \\
\rowcolor[HTML]{D1D1D1} 
Lamda (GAE)                 & 0.95           \\
\rowcolor[HTML]{EFEFEF} 
Worker Steps                & 512            \\
\rowcolor[HTML]{D1D1D1} 
Minibatches                 & 8              \\
\rowcolor[HTML]{EFEFEF} 
$c_1$                        & 0.25           \\
\rowcolor[HTML]{D1D1D1} 
Max Gradient Norm           & 0.5            \\
\rowcolor[HTML]{EFEFEF} 
Clip Range                  & 0.2            \\
\rowcolor[HTML]{D1D1D1} 
Hidden State Size           & 512            \\
\rowcolor[HTML]{EFEFEF} 
Recurrent Layer             & GRU            \\
\rowcolor[HTML]{D1D1D1} 
Sequence Length             & Max            \\
\rowcolor[HTML]{EFEFEF} 
Activations                 & ReLu           \\
\rowcolor[HTML]{D1D1D1} 
Optimizer                   & AdamW         
\end{tabular}
\caption{Shared parameters used for training.}
\label{tab:common}
\end{small}
\end{table}

==> tables/config_specific.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{small}
\centering
\begin{tabular}{l|rrr}
\rowcolor[HTML]{D1D1D1} 
\textbf{Parameter} & \multicolumn{1}{c}{\cellcolor[HTML]{D1D1D1}\textbf{Mortar}} & \multicolumn{1}{c}{\cellcolor[HTML]{D1D1D1}\textbf{Spotlights}} & \multicolumn{1}{c}{\cellcolor[HTML]{D1D1D1}\textbf{Ballet}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
Seeds              & 1000                                                    & 1000                                                            & 500                                                         \\
\rowcolor[HTML]{D1D1D1} 
Visual Obs.        & 84x84x3                                                 & 84x84x3                                                         & 99x99x3                                                     \\
\rowcolor[HTML]{EFEFEF} 
Vector Obs.        & 490+4+1                                                 & 6+1                                                             & 13+8+1                                                      \\
\rowcolor[HTML]{D1D1D1} 
Action Space       & 4                                                       & 3, 3                                                            & 8                                                           \\
\rowcolor[HTML]{EFEFEF} 
Vector FC Size    & 256                                                     & 128                                                             & 128                                                         \\
\rowcolor[HTML]{D1D1D1} 
Num. Workers       & 32                                                      & 16                                                              & 32                                                          \\
\rowcolor[HTML]{EFEFEF} 
Batch Size         & 16384                                                   & 8192                                                            & 16384                                                       \\
\rowcolor[HTML]{D1D1D1} 
Epochs             & 4                                                       & 3                                                               & 3                                                           \\
\rowcolor[HTML]{EFEFEF} 
Initial $\alpha$      & 0.0003                                                  & 0.0003                                                          & 0.0003                                                      \\
\rowcolor[HTML]{D1D1D1} 
Min $\alpha$          & 0.00003                                                 & 0.0003                                                          & 0.0003                                                      \\
\rowcolor[HTML]{EFEFEF} 
Initial $c_2$       & 0.1                                                     & 0.0001                                                          & 0.001                                                       \\
\rowcolor[HTML]{D1D1D1} 
Min $c_2$           & 0.0001                                                  & 0.0001                                                          & 0.0005                                                     
\end{tabular}
\caption{Individual parameters used for training.
Vector observations combine the original observation, the agent's last action (one-hot) and reward.
The learning rate $\alpha$ and $c_2$ decay linearly.
Vector FC Size denotes the size of the fully connected layer used to encode the vector observation.}
\label{tab:specific}
\end{small}
\end{table}
